Model Compression Techniques in Biometrics Applications: A Survey

The development of deep learning algorithms has extensively empowered humanity's task automatization capacity. However, the huge improvement in the performance of these models is highly correlated with their increasing level of complexity, limiting their usefulness in human-oriented applications, which are usually deployed in resource-constrained devices. This led to the development of compression techniques that drastically reduce the computational and memory costs of deep learning models without significant performance degradation. This paper aims to systematize the current literature on this topic by presenting a comprehensive survey of model compression techniques in biometrics applications, namely quantization, knowledge distillation and pruning. We conduct a critical analysis of the comparative value of these techniques, focusing on their advantages and disadvantages and presenting suggestions for future work directions that can potentially improve the current methods. Additionally, we discuss and analyze the link between model bias and model compression, highlighting the need to direct compression research toward model fairness in future works.

==> sections/not_used/bias_notused.tex <==
\section{Bias} \label{sec:bias}

% I would remove this due to the reframing of the "Bias" section

% One way to assess whether global metrics are truly representative of the verified losses in performance is by analyzing the samples whose classification is negatively influenced by these losses. This can be done by determining how these samples are distributed over the categories present in the testset. If this distribution of categories is similar to the one verified in the whole testset, the global metrics produce a good representation of the performance loss introduced by model compression. However, distribution shifts indicate that the compressed model is neglecting specific types of samples, resulting in the introduction of an undesired bias. 



% ------

%Wang~\textit{et al.}~\cite{wang2019racial} proposed the Racial Faces in the Wild (RFW) dataset, which contains equal percentages of faces from Caucasian, Indian, Asian and African identities. Since pre-trained FR models showed a strong tendency to prioritize the correct classification of Caucasian pairs, an alternative well-balanced train dataset was also proposed. Models trained on this dataset have reduced racial bias, but they still perform better for Caucasian faces, since non-Caucasian faces have characteristics that might be harder to extract and preprocess, especially in a dark acquisition environment. 

%Following a similar line of thought, Karkkainen~\textit{et al.}~\cite{karkkainen2021fairface} addressed the debiasing of the gender classification task by proposing FairFace, a race-balanced dataset that is diverse in terms of race, age, expressions, head orientation, and photographic conditions. The races are split into 7 categories, allowing for further separation between races that share common features but are still easily distinguishable: White, Black, Indian, EastAsian, Southeast Asian, Middle Eastern, and Latino. Models trained with FairFace achieved generally higher accuracies and more consistent performances between the evaluated races, as proved by the lower standard deviation between the accuracies of the 7 races. As such, using well-balanced training data is important to reduce the racial bias of a model.

%Robinson~\textit{et al.}~\cite{robinson2020face} presented Balanced Faces in the Wild (BFW), a balanced FR dataset in terms of race, gender and race+gender to analyze the way the performance of FR models is usually evaluated. Generally, an FPR value is fixed and, based on that value, the model establishes a threshold that separates the different identities in an angular way. The authors show that using the same threshold for all identities leads to different FPR and FNR values associated with which subgroup, meaning that some of these subgroups attain a higher FPR value than the defined goal, which is undesired. Hence, they define a set of thresholds that are applied to each race/gender pair and operate under the same FPR value. Although this approach resulted in an improved TAR for all the tested subgroups, this improvement was poor for low FAR values. Besides, this study lacks a well-supported analysis of how this technique contributes to reducing the bias of the network. Despite having calculated all the TAR values, no metric is used to perform a comparison with the baseline. As such, a deeper performance analysis should be conducted. 

%%Wang~\textit{et al.}~\cite{wang2021meta} proposed two novel training sets: BUPT-Globalface follows the real-world skin-tone distribution and BUPT-Balancedface is balanced in equal proportions among all the considered skin-tones. Models trained with different loss functions performed better when trained on these datasets, especially on BUPT-Balancedface, confirming that data-related bias can be reduced by using well-balanced training datasets. However, contrary to what the authors suggest, BUPT-Globalface and BUPT-Balancedface do not follow a similar distribution across different skin tones. As an example, Tone-III and Tone-VIII have about 45\% and 5\% of females respectively. Attributes such as gender should also be well-balanced, but female identities are severely underrepresented. Although this is not easy to achieve, benchmarks that are well-balanced regarding several sensitive attributes and not only one should be developed. Ignoring this need might result in models that are unbiased regarding the characteristic they are being analyzed for (race, in this case) while withholding increased bias regarding other sensitive attributes (such as gender), as will be discussed later in Section \ref{sec:impact}.  

==> sections/not_used/not_used.tex <==

% Despite being widely deployed in Biometrics applications, the possible application scenarios of KD are not restricted to this field. \cite{beyer2022knowledge} utilized a simple RB-KD loss to identify the best way to distill knowledge between a teacher and a student in CV tasks such as flowers and food classification. They concluded that it is possible to obtain models with top performance by combining aggressive data augmentation with extensive training. Aggressive data augmentation increases the size of the dataset by the addition of mixtures of images from completely different scenarios, which helps reduce overfitting and obtain more generalizable models. When combined with extremely lengthy training procedures (about 1 million epochs with a batch size of 500 for the flower classification task), this strategy results in students that reach the same performance as the teacher networks, shedding some light on how to achieve SOTA results with KD-compressed models. However, these extremely long training procedures are generally not feasible, invalidating the proposed method, which generally performs worse than common KD methodologies when the number of training epochs is lower. 

%Most of the current KD studies present results that are obtained by using the same dataset to train the teacher and the student networks. However, there is no guarantee that the dataset used to train the original teacher network is publicly available for further training, namely due to privacy reasons, compromising the standard KD procedure. To address this problem, \cite{choi2020data} used the representations embedded in the teacher network to train a GAN that generates approximations of the teacher's input images, which are then used to feed the student model. The latter is trained simultaneously with the GAN, employing a response-based KL divergence loss term. The obtained network achieved SOTA performance among the available data-free approaches, but it still fell behind a student trained from scratch using the original data. They also proved that the KD step contributes to enhancing the performance of a quantized model trained with the GAN-generated images. However, it should be noted that this study lacks the analysis of FB-KD under similar circumstances, which could also lead to competitive results.

%\cite{hinton2015distilling} transferred knowledge from an ensemble of teachers to a single student following an SRB-KD approach. The authors prove that it is possible to transfer the generalization capabilities of the ensemble to a single student for both number identification and speech recognition tasks. However, they do not limit their conclusions to model compression, showing that KD can be used to enhance models with other types of restraints, namely regarding the amount of available training data. Using KD to transfer the teachers' knowledge to a student that only had access to 3\% of the original dataset resulted in lower performance drops than the ones verified by a student trained from scratch with the same small dataset. Similar results were obtained when training the student network with the samples belonging only to some of the classes present on the dataset. Both situations derive from the fact that the teacher was trained using a more complete set of data, meaning that approximating its soft probability space might result in an implicit understanding of the missing samples' classification, dampening the overfitting effect. 

% I decided that this one is not that interesting after all
While studying a concept for the first time, human learners often misunderstand some details that are later clarified when approaching more complex issues. Considering this characteristic of the human learning process, Chen~\textit{et al.}~\cite{chen2021distilling} proposed an interesting approach based on the distillation of knowledge from different points of the teacher to each posterior layer of the student. The information encoded by the teacher in previous layers can contribute to the learning process of higher-level student layers, allowing the student to review previously learned concepts (lower-level features) and understand them deeply while evolving in the learning process. The fact that humans cannot understand complex concepts without first understanding their basic fundamentals explains why the process is not reversed, that is, why the student layers do not learn from subsequent teacher layers. Since the knowledge is being transferred from between differently sized layers, there is the need to use several adaption functions between the teacher and the student, which poses a disadvantage. The authors tested their approach in image classification, object detection and instance segmentation tasks, achieving decent results in all of the analyzed scenarios. 

% One of the biggest problems associated with DNNs is their lack of interpretability, which is generally associated with their complexity degree and also with the fact that their inner working is unknown. Nowadays, interpretability is a very important research focus, namely due to the fact that it is essential in situations such as critical-risk scenarios, like medical applications. Despite being commonly applied between a pair of DNNs, \cite{liu2018improving} used SRB-KD to transfer knowledge between a pretrained DNN and the output of a decision tree, which is inherently interpretable by humans. This output is then passed through a softmax layer to obtain the final decision tree soft targets, which are used to predict the class of each input sample. KD-based decision trees achieved performances up to 5 percentual points superior than non-KD decision trees. The achieved results are presented for various depth limits and the trees that are more deeply expanded present better performances, as expected. However, it should be kept in mind that the absence of a reasonable depth limit leads to results that cannot be properly interpreted by a human agent, which goes against the purpose of the current method. Using an appropriate search depth leads to a student decision tree whose performance stays far behind the one achieved by the teacher DNN. More studies should be conducted in this field to boost the development of inherently interpretable models that match the currently used DNNs in terms of performance.

%\cite{han2023impact} also focused on verifying whether KD can be used to improve model interpretability, by comparing an object classification model trained from scratch, a version trained with KD and a third version trained with label smoothing (LS). LS is similar to RB-KD but it uses a uniform distribution as the proxy, meaning that the model is trained with the usual cross-entropy loss and with an extra term that considers equal probabilities for each class. It should be noted that this does not account for a class-similarity separation that can be useful for interpretability purposes and that is generally present when KD is used. The interpretability of these models was tested using several metrics that led to similar conclusions, namely the number of concept detectors, GT heatmaps of a synthesized dataset, DiffROAR scores and loss gradients. As an example, models trained with KD presented a larger number of concept detectors, proving that KD can improve model interpretability. In this scenario, the improvement in the number of object detectors should be highlighted since it proves that KD allowed the model to focus more on the identified objects, enhancing its interpretability. On the other hand, the usage of LS reduced the number of object detectors, generating activation maps that enhance the background areas of the image, as it forces the model to learn all the classes by giving them equal probabilities. Hence, while both KD and LS performed better than the baseline (with KD achieving higher accuracy), only KD improved the interpretability of the model since it transfers a higher amount of class-similarity information to the student model, promoting an easier interpretation by the human observer. Furthermore, adding RB-KD to FB-KD improved the interpretability of the final model since logits contain more class-similarity information than features extracted from the middle of the network, proving that the usage of RB-KD can be helpful and shouldn't be disregarded.
